Fundamental bounds on many-body spin cluster intensities

Multiple-quantum coherence (MQC) spectroscopy is a powerful technique for probing spin clusters, offering insights into diverse materials and quantum many-body systems. However, prior experiments have revealed a rapid decay in MQC intensities as the coherence order increases, restricting observable cluster sizes to the square root of the total system size. In this work, we establish fundamental bounds on observable MQC intensities in the thermodynamic limit outside the weak polarisation limit. We identify a sharp transition point in the observable MQC intensities as the coherence order grows. This transition points fragments the state space into two components consisting of observable and unobservable spin clusters. Notably, we find that this transition point is directly proportional to the size $N$ and polarization $p$ of the system, suggesting that the aforementioned square root limitation can be overcome through hyperpolarization techniques. Our results provide important experimental guidelines for the observation of large spin cluster phenomena.

==> symbols/main.tex <==
\input symbols/symbols.tex
\input symbols/refgroups.tex

==> symbols/symbols.tex <==
\DeclareMathAlphabet{\mymathbb}{U}{BOONDOX-ds}{m}{n}

%%  group theory
\newcommand\SN{{\rm S}_{n}}
\newcommand\AN{{\rm A}_{n}}
\newcommand\Athree{{\rm A}_{3}}
\newcommand\Sthree{{\rm S}_{3}}
\newcommand\Stwo{{\rm S}_{2}}
\newcommand\Cthree{{\rm C}_{3}}
\newcommand\UN{{\rm U}(n)}
\newcommand\SUN{{\rm SU}(n)}
\newcommand\SOthree{{\rm SO}(3)}
\newcommand\SOtwo{{\rm SO}(2)}

%%  parameters
\newcommand\wL{\omega_{0}}

%%  operator
\newcommand\one{\mathbbm{1}}
\newcommand\zero{\mymathbb{0}}
\newcommand\boldI{{\bf I}}
\newcommand{\Hop}{\mathcal{H}}
\newcommand{\Hcoh}{\Hop_{\rm coh}}

%%  group theory
\newcommand\spart[1]{{[}#1{]}}
\newcommand\Wtilde[1]{\stackrel{\sim}{\smash{#1}\rule{0pt}{1.5ex}}}
\newcommand\Wtildeb[1]{\stackrel{\sim}{\smash{#1}\rule{0pt}{1.1ex}}}
%%  relaxation
\newcommand{\Tone}{T_{1}}
\newcommand{\Ttwo}{T_{2}}

%%  math symbols
\newcommand{\iu}{{i\mkern1mu}}
\newcommand\myeq[1]{\stackrel{\mathclap{\normalfont\mbox{#1}}}{=}}

% -- Hilbert space --
\newcommand\NH{N_{\mathcal{H}}}
\newcommand\ket[1]{|#1\rangle}
\newcommand\bra[1]{\langle#1|}
\newcommand\braket[2]{\left<#1|#2\right>}
\renewcommand\a{\alpha}
\renewcommand\b{\beta}

% -- Liouville space --
\newcommand\Ket[1]{|#1)}
\newcommand\Bra[1]{(#1|}
\newcommand\BraKet[2]{(#1|#2)}
\newcommand{\Lop}{\mathcal{L}}
\newcommand\Lzero{\hat{\Lop}_{\rm coh}}
\newcommand\Relax{\hat{\mathcal{R}}}

%
\newcommand\CBnote[1]{\textcolor{orange}{[#1]}}
\newcommand\CZWnote[1]{\textcolor{blue}{[#1]}}

% -- columns--
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{?}{!{\vrule width 1pt}}
